Collecting a Large-Scale Gender Bias Dataset for Coreference Resolution and Machine Translation

Recent works have found evidence of gender bias in models of machine translation and coreference resolution using mostly synthetic diagnostic datasets. While these quantify bias in a controlled experiment, they often do so on a small scale and consist mostly of artificial, out-of-distribution sentences. In this work, we find grammatical patterns indicating stereotypical and non-stereotypical gender-role assignments (e.g., female nurses versus male dancers) in corpora from three domains, resulting in a first large-scale gender bias dataset of 108K diverse real-world English sentences. We manually verify the quality of our corpus and use it to evaluate gender bias in various coreference resolution and machine translation models. We find that all tested models tend to over-rely on gender stereotypes when presented with natural inputs, which may be especially harmful when deployed in commercial systems. Finally, we show that our dataset lends itself to finetuning a coreference resolution model, finding it mitigates bias on a held out set. Our dataset and models are publicly available at www.github.com/SLAB-NLP/BUG. We hope they will spur future research into gender bias evaluation mitigation techniques in realistic settings.

==> sections/2-background.tex <==
\section{Background}
In this work we follow \citet{stanovsky-etal-2019-evaluating} work who created an automatic gender bias evaluation method that estimates the performance of machine translation models on translating correctly from English into languages with grammatical gender the information about gender of an entity in a sentence.
They evaluated the difference of the performance of the models between masculine and feminine scores, and between pro-stereotypical and anti-stereotypical gender role assignments and showed machine translation models are significantly prone to translate based on gender stereotypes. This work limitation is that the test set they used includes syntactic sentences with very simple structure. The distribution of this set differs from that on which the machine translation systems were trained on, so it could be that the gender bias found in the evaluation is artificial and we won’t find it in sentences from natural text. Other than this, the medium size test set (3888 sentences), can be overfit.





==> sections/9-conclusion.tex <==
\section{Conclusion}
We presented in this work the BUG corpus, a large-scale (108K) corpus of diverse real-world English sentences, collected by semi-automatic grammatical search of patterns indicating stereotypical and anti-stereotypical gender-role assignments.
Using BUG, we evaluated gender bias in various coreference resolution and machine translation models, and found that all tested models tend to translate and associate entities with accordance to gender stereotypes, even when in conflict with opposite gendered pronouns in the sentence.
After doing so, we showed the feasibility of training with our corpus by finetuning a coreference resolution model on it, finding it improves performance on a held out set.
Our data and code are publicly available at \url{\repolink}.

